Stacking and Registry Effects in Layered Materials: The Case of Hexagonal Boron Nitride

The interlayer sliding energy landscape of hexagonal boron nitride (h-BN) is investigated via a van der Waals corrected density functional theory approach. It is found that the main role of the van der Waals forces is to "anchor" the layers at a fixed distance, whereas the electrostatic forces dictate the optimal stacking mode and the interlayer sliding energy. A nearly free-sliding path is identified, along which bandgap modulations of ~0.6 eV are obtained. We propose a simple geometrical model that quantifies the registry matching between the layers and captures the essence of the corrugated h-BN interlayer energy landscape. The simplicity of this phenomenological model opens the way to the modeling of complex layered structures, such as carbon and boron nitride nanotubes.

==> Makefile <==
.SUFFIXES: $(SUFFIXES) .dvi .ps .bib .tex .bbl .pdf

    PAPER_ROOT = hBN

  AIX_PSVIEWER = ghostview
Linux_PSVIEWER = ghostview
SunOS_PSVIEWER = ghostview

INFILES =  hBN.tex \
#	fkt.eps \
#	skw.eps


# PICTURES = 
#
# A very cool hack to "do the right thing":
       PSVIEWER = ${$(OS)_PSVIEWER}
#
#
# standard rules:
#
.dvi.ps:
	touch $*.ps
	/bin/rm $*.ps
	@echo "compiling $*"
	dvips -t a4 -o $*.ps $<

.ps.pdf:
	touch $*.pdf
	/bin/rm $*.pdf
	@echo "compiling $*"
	ps2pdf $< $*.pdf 

all:: ${PAPER_ROOT}.view

outline:: ${OUTLINE}.view

gs:: ${PAPER_ROOT}.psview

print: ${PAPER_ROOT}.ps  ${PAPER_ROOT}.pdf
print_outline: ${OUTLINE}.ps
	lpr ${OUTLINE}.ps

${PAPER_ROOT}.dvi: ${INFILES} ${PAPER_ROOT}.bib ${PICTURES}
	latex ${PAPER_ROOT}
	bibtex ${PAPER_ROOT}
	latex ${PAPER_ROOT}
	latex ${PAPER_ROOT}

${OUTLINE}.dvi: ${OUTLINE}.tex ${OUTLINE}.bib ${PICTURES}
	latex ${OUTLINE}
	bibtex ${OUTLINE}
	latex ${OUTLINE}
	latex ${OUTLINE}
	chmod 664 ${OUTLINE}.blg ${OUTLINE}.bbl ${OUTLINE}.aux ${OUTLINE}.dvi ${OUTLINE}.log

${PAPER_ROOT}.psview: ${PAPER_ROOT}.ps
	${PSVIEWER} ${PAPER_ROOT}.ps

${PAPER_ROOT}.view: ${PAPER_ROOT}.dvi
	xdvi ${PAPER_ROOT}

${OUTLINE}.view: ${OUTLINE}.dvi
	xdvi ${OUTLINE}

clean::
	/bin/rm -f *.aux *.log *.bbl *.blg *.dvi *~



